Verdier quotients of Calabi-Yau categories from quivers with potential

We study a class of triangulated categories obtained as Verdier quotients of 3-Calabi-Yau categories combinatorially described by quivers with potential from (decorated) marked surfaces. We study their bounded t-structures and consider in particular the exchange graphs of hearts and silting objects, and show that the Koszul isomorphism between these graphs is preserved under Verdier quotient.

==> packages.tex <==

%languages, pictures
\ProvidesPackage{language}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{csquotes}
\usepackage{graphicx,color}
\usepackage[colorlinks, linkcolor=blue!50,anchorcolor=Periwinkle,
citecolor=blue!72,urlcolor=cyan, bookmarksopen,bookmarksdepth=2]{hyperref}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{anyfontsize}
\usepackage{comment}
% for list of notation
\usepackage{array}
\usepackage{hang}
\setlength{\hangingindent}{2em}

%biblatex
%\usepackage[style=alphabetic,backend=bibtex,maxnames=10]{biblatex}
\usepackage[style=alphabetic,
            isbn=false,
            doi=false,
            url=false,
            backend=bibtex,
            maxnames=5,
            maxalphanames=5,firstinits=true
           ]{biblatex}
%\usepackage{layout}
\usepackage{enumitem}
\usepackage{afterpage}
%\usepackage{parskip}
\usepackage{aliascnt}
%\usepackage[notref,notcite]{showkeys}
\usepackage{xparse}
\usepackage{caption}
%\usepackage{tabto}
\usepackage{imakeidx}
%\usepackage[normalem]{ulem}
\allowdisplaybreaks


%math
\usepackage{amsmath,amsfonts,amsthm,mathtools,amssymb}
\usepackage{tensor}
\usepackage{amscd,latexsym, mathrsfs, epsfig}
\usepackage{mathdots}
\usepackage{upgreek}
%\usepackage{enumerate}
%\usepackage{undertilde}
\usepackage[all]{xy}
%\usepackage{transparent}
%tikz
\usepackage{tikz}
\usepackage{pgf,tikz-3dplot}
\usepackage{tikz-cd}
\usepackage{float}
\usepackage{circuitikz}
\usetikzlibrary{positioning}
\usetikzlibrary{matrix, calc, arrows, decorations.pathreplacing, decorations.markings, decorations.pathmorphing, backgrounds,fit,positioning,shapes.symbols,chains,shadings,fadings}
\usetikzlibrary{cd}
\usetikzlibrary{intersections}
\tikzset{
	every loop/.style={very thick},
	comp/.style={circle,black,draw,thin,inner sep=0pt,minimum size=5pt,font=\tiny},
	order bottom left/.style={pos=.05,left,font=\tiny},
	order top left/.style={pos=.9,left,font=\tiny},
	order bottom right/.style={pos=.05,right,font=\tiny},
	order top right/.style={pos=.9,right,font=\tiny},
	%
	order middle right/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,right,font=\tiny},
	%
	order middle left/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,left,font=\tiny},
	%	
	order node dis/.style={text width=.75cm},
	circled number/.style={circle, draw, inner sep=0pt, minimum size=12pt},
	below left with distance/.style={below left,text height=10pt},
	below right with distance/.style={below right,text height=10pt}
}

\tikzset{->-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{>}}},postaction={decorate}}}
\tikzset{-<-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{<}}},postaction={decorate}}}
\tikzset{%
glow/.style={%
preaction={#1, draw, line join=round, line width=0.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=1.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=1.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=2.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=2.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=3.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=3.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=4.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=4.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=5.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=5.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=6.0pt, opacity=0.04,
}}}}}}}}}}}}}}
